Grid-based state space exploration for molecular binding

Binding processes are difficult to sample with molecular-dynamics (MD) simulations. In particular, the state space exploration is often incomplete. Evaluating the molecular interaction energy on a grid circumvents this problem but is heavily limited by state space dimensionality. Here, we make the first steps towards a low-dimensional grid-based model of molecular binding. We discretise the state space of relative positions and orientations of the two molecules under the rigid body assumption.The corresponding program is published as the Python package molgri. For the rotational component of the grids, we test algorithms based on Euler angles, polyhedra and quaternions, of which the polyhedra-based are the most uniform. The program outputs a sequence of molecular structures that can be easily processed by standard MD programs to calculate grid point energies. We demonstrate the grid-based approach on two molecular systems: a water dimer and a coiled-coil protein interacting with a chloride anion. For the second system we relax the rigid-body assumption and improve the accuracy of the grid point energies by an energy minimisation. In both cases, oriented bonding patterns and energies confirm expectations from chemical intuition and MD simulations. We also demonstrate how analysis of energy contributions on a grid can be performed and demonstrate that electrostatically-driven association is sufficiently resolved by point-energy calculations. Overall, grid-based models of molecular binding are potentially a powerful complement to molecular sampling approaches, and we see the potential to expand the method to quantum chemistry and flexible docking applications.

==> attic.tex <==
\section{Attic}

\textbf{Open source.}
...anybody with a Python installation can quickly access, test and modify the code we implemented. We believe that the availability of well-documented, open-source code adds an extra layer of transparency and repeatability to the method we are proposing. We also hope that the presence of integrated as well as compiled documentation and a publicly visible version-controlled source code with issue tracking encourages discussion and collaboration.\\

\medskip
\textbf{Convergence of coverage.}
Before they can be used to generate pseudotrajectories, the sphere grids need to be tested on two accounts: (i) the convergence of coverage, i.e is every area on the sphere sampled as $N \rightarrow \infty$ and (ii)  the uniformity of coverage, i.e. are any two areas of the same size sampled with equal probability. \bk{[Moved from above.]}

As a final step we take a closer look at the speed of convergence. For this purpose, consider another important measure called \textit{arch distance}. To obtain it, we first randomly position 500 points on the surface of the sphere and then for each of them find the closest grid point, measuring the length of the spherical arch connecting them. This is the arch distance. Over the sample of 500 points, we can compute the average distance of a random point to the closest grid point for different sampling algorithms and different $N$s. Since this method does not use ratios, we can observe how quickly the values converge for large $N$s, i.e. how quickly the average coverage level doubles. In \figref{convergence_arch} we plot the $y \propto x^{-2}$ line on a log-log plot to indicate that most algorithms (icosahedron, cube 3D, random quaternion and random Euler angles grids) are parallel to this line and therefore converge with the same speed. This means that by doubling the number of points, the average distance to a grid point reduces for a factor of 4, quickly improving coverage. The systematic Euler and cube 4D algorithms underperform in this regard, converging more slowly than the competing algorithms.

\medskip
\textbf{Convergence of coverage.}
All in, we can conclude that all used algorithms replicate theoretically expected coverage values for large numbers of points; however, most have difficulty achieving uniformity when comparing small areas at different portions of the sphere. Polyhedra-based grids, in our case the 3D cube and icosahedron grid, show excellent results on all fronts: they have remarkably small variance in coverages regardless of the alpha and axis selected; they are the first to converge to theoretically predicted coverages and have on average the shortest distance between a random point and the nearest grid point of all tested algorithms. Somewhat longer generation times are well worth the improved quality. We recommend their use for rotation sampling and use icosahedron grid as our method of choice in subsequent applications.

\medskip
\textbf{Convergence of coverage.}
In \figref{convergence_alpha}, we plot the average coverage $N_{sc}/N$ (again averaging over 100 directions) for $N$s ranging from 3 to 1000. We use the same range of values for $\alpha$ ($\pi/6$ to $5\pi/6$) and colour-code them in the same way as in \figref{violin_alpha}. In addition, we plot the theoretical limits $A_{sc}/A_{sphere}$ given by \equref{ideal_ratio} as black lines. We observe that all algorithms converge towards the theoretical limit for larger alphas while systematic Euler, random Euler and 4D cube algorithm tend to somewhat underestimate the expected value for the smallest angle $\alpha=\pi/6$, suggesting a systematic bias in the generation algorithm. 3D cube and icosahedron grid converge particularly quickly. At only $N=100$ the 3D cube algorithm already differs just 0.7\% and the icosahedron one 0.1\% from the theoretical value for the $\alpha=\pi/6$ example, even less for the rest of the angles.\\

Now we expect two properties from an optimal grid: (i) for large $N$, the ratio of $N_{sc}/N$ should approach the theoretical limit $A_{sc}/A$ for each $\alpha$ and each axis, and (ii) the variance of $N_{sc}/N$ with regard to different selections of axes should be minimal.

% \begin{figure}
%     \centering
%     \includegraphics[width=\textwidth]{images/_panel_alpha_con.pdf}
%     \caption[Convergence of grid coverages to theoretical values]{Convergence of coverages $N_{sc}/N$ (coloured lines) to the theoretical values $A_{sc}/A$ (black lines) for angles $\pi/6$ (red), $2\pi/6$ (lime green), $3\pi/6$ (dark green), $4\pi/6$ (blue) and $5\pi/6$ (violet). Plotted is the coverage averaged over 100 random axes along with the 95\% confidence interval. We observe convergence to expected values for large $Ns$ with some systematic deviations for $\alpha=\pi/6$; 3D cube and icosahedron grid converge particularly quickly.}
%     \label{fig:convergence_alpha}
% \end{figure}

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.8\textwidth]{images/convergence_SD.pdf}
%     \caption[Speed of convergence for grid algorithms]{Arch distance to the closest grid point is measured for 500 random points on a unit sphere and averaged. Dotted line indicates the $y = x^{-2}$ relationship. Arch distance decreases with the number of grid points, speed of the decrease indicates the speed of convergence. The cube 3D and icosahedron algorithms as well as both random algorithms are essentially indistinguishable in this metric; all converge at the rate of $y \propto x^{-2}$ (although random algorithms start at a higher value). Systematic Euler and cube 4D algorithms converge slower than $y \propto x^{-2}$. The graph of standard deviations of arch distances shows the same trends.}
%     \label{fig:convergence_arch}
% \end{figure}



\medskip
\textbf{Computational cost: coiled-coil}
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.8\textwidth]{images/protein0_CL_ico_100000_full_pot_conv.pdf}
    \caption[hFF03-Cl$^-$, calculation time]{hFF03-Cl$^-$: minimal potential energy found in pseudotrajectories of different lengths (sampled translations remain the same, density of rotation sampling changes) and runtime of calculations. }
    \label{fig:hFF03-Cl_time} %The computational time plotted with dashed lines includes the GROMACS run and saving the results in a standard format for an MD run and a pseudotrajectory generation, GROMACS re-run and saving in a standard format for an icosahedron run.
\end{figure}



\medskip
\textbf{Set-up for the coiled-coil system}

\begin{figure}[h!]
    \centering
    \begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=0.7\textwidth]{images/protein0_double.pdf}
    \end{subfigure}%
    \hfill
    \begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=\textwidth, trim={0 2.5cm 0 2.5cm},clip]{images/set_up_30_full.pdf}
    \end{subfigure}
    \caption[Structure of hFF03 and an example of pseudotrajectory set-up.]{Left: molecular structure of the hFF03 polypeptide. Right: example of a pseudotrajectory ($N=30$, distances 0.5 - 2.5 nm) with a probe Cl$^-$ ion shown in yellow. Atoms are drawn as spheres using the van der Waals radii of individual elements and a standard colouring scheme (black for carbon, white for hydrogen, red for oxygen and blue for nitrogen).}
    \label{fig:protein0}
\end{figure}


\textbf{Coiled-coil peptide and Cl$^-$ vs Na$^+$}
When plotting 100 frames, an interesting difference between the positive and negative ion case is the strong localisation of the low-energy Na$^+$ structures and the larger spread of Cl$^-$ low-energy structures. This is probably the consequence of the protein having the charge +7 in the set-up of the simulation (physiological pH), resulting in a strong attraction of the chlorine ion to hFF03. Nevertheless, it would be interesting to examine in self-assembly studies whether branching of the hFF03 networks occurs primarily on positively charged side groups, which is what the \figref{protein0_Cl_Na_100} would predict.\\

\textbf{Computational cost: coiled-coil}
Energy minimisation largely occurs due to those conformation changes and not due to protein-ion interaction. In real trajectories with up to 10$^5$ time steps the ion barely moves from the initial state if it is chosen appropriately while a pseudotrajectory tests the entire range of orientations and distances in this time. Due to this large difference in sampled motion we omit direct comparison of energies but still compare (pseudo)trajectories in their computational times in \figref{hFF03-Cl_time}. For this system with $\approx 1000$ atoms, pseudotrajectory calculations are faster than MD calculations from about 10$^4$ trajectory points on.


\textbf{Proof of concept}
 We consider the test systems presented to be a proof of concept that grid-based approaches to association can provide relevant information about molecular systems using only a small number of energy calculations and avoiding any re-sampling of minima. 
 
 
 
 \textbf{Modules within \texttt{molgri}}
 For advanced users who may prefer to use \texttt{molgri} as a python package and enjoy more flexibility, the package is easily imported as \texttt{import molgri}. A quick overview of modules provided in the package is as follows:

\begin{lstlisting}[style=DOS]
molgri/
 |-wrappers.py   timing other functions
 |-analysis.py   analysing uniformity and convergence
 |-bodies.py     applying rotations and translations on 3D objects
 |-grids.py      abstract object Grid and derived rotation grid types
 |-parsers.py    interpreting grid types and .gro files
 |-paths.py      references to current input/output directories
 |-pts.py        Pseudotrajectory object and generation of .gro files
 |-rotations.py  rotation set <-> grid transformations
 |-constants.py  package-related constants
 |-plotting.py   various plot and animation types
 \end{lstlisting}



The field of theoretical chemistry is continuously trying to learn more about molecular behaviour while simultaneously minimising computational costs. A big obstacle on the way to this goal is the nature of configuration space, consisting of narrow low-energy areas divided by high and complex barriers. In unbiased MD simulations, the time spent in an area has an inverse exponential relationship with the energy of this state, rendering escapes out of deep minima extremely rare events. As a consequence, the vast majority of computational time is spent on re-examining the same minima over and over again.

